From Blind Solvers to Logical Thinkers: Benchmarking LLMs' Logical Integrity on Faulty Mathematical Problems

Consider the math problem: "Lily received 3 cookies from her best friend yesterday and ate 5 for breakfast. Today, her friend gave her 3 more cookies. How many cookies does Lily have now?" Many large language models (LLMs) in previous research approach this problem by calculating the answer "1" using the equation "3 - 5 + 3." However, from a human perspective, we recognize the inherent flaw in this problem: Lily cannot eat 5 cookies if she initially only had 3. This discrepancy prompts a key question: Are current LLMs merely Blind Solver that apply mathematical operations without deeper reasoning, or can they function as Logical Thinker capable of identifying logical inconsistencies? To explore this question, we propose a benchmark dataset, FaultyMath, which includes faulty math problems of rich diversity: i) multiple mathematical categories, e.g., algebra, geometry, number theory, etc., ii) varying levels of difficulty, and iii) different origins of faultiness -- ranging from violations of common sense and ambiguous statements to mathematical contradictions and more. We evaluate a broad spectrum of LLMs, including open-source, closed-source, and math-specialized models, using FaultyMath across three dimensions: (i) How accurately can the models detect faulty math problems without being explicitly prompted to do so? (ii) When provided with hints -- either correct or misleading -- about the validity of the problems, to what extent do LLMs adapt to become reliable Logical Thinker? (iii) How trustworthy are the explanations generated by LLMs when they recognize a math problem as flawed? Through extensive experimentation and detailed analysis, our results demonstrate that existing LLMs largely function as Blind Solver and fall short of the reasoning capabilities required to perform as Logical Thinker.

==> 1introduction.tex <==
\section{Introduction}

%In many classroom settings, particularly during exams, teachers sometimes present students with math problems that contain unintentional mistakes or inconsistencies. Students often quickly recognize these errors, understanding that the problem, as stated, cannot be solved without modification—an ability that is a fundamental aspect of mathematical reasoning. But what happens when such a scenario is presented to advanced Artificial Intelligence, particularly Large Language Models (LLMs)? These models have revolutionized areas ranging from machine-translation to complex problem-solving \cite{brown2020language, openai2023gpt4, hendrycks2021measuring} and excel at tackling intricate mathematical problems. But can they, with all their advancements, similarly identify and reason through unsolvable problems in mathematics?

\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth]{figures/false_math_example_from_dataset.pdf} 
\caption{Example of a ``False Math Problem" from our dataset. The model responses are their final numerical output after reasoning.}
\label{fig:false_math_problem_example}
\end{figure}

While LLMs like GPT-4 and Gemini-1.5-Pro have demonstrated remarkable abilities in solving intricate mathematical problems \citep{brown2020language, openai2023gpt4, hendrycks2021measuring} when presented with solvable ones, their skill in a more nuanced challenge—identifying inherently false math problems—has been less studied. An example is shown in Figure \ref{fig:false_math_problem_example}. A simple system of equations with two unknowns should resolve the problem easily; however, it results in a negative cost for either feathers or gold, which defies common sense. Despite this, three LLMs provided answers without recognizing the error in their analysis.

A math problem is considered false and unsolvable if it cannot be solved without altering the problem statement. Humans recognize the unsolvability of such problems based on the nature and complexity of the question. This research investigates whether LLMs can meet this challenge by exploring the limits of their logical reasoning and assessing their ability to detect unsolvable problems.

The primary challenge in this research was creating a diverse dataset of false math problems spanning different difficulty levels, various mathematical categories (such as algebra, geometry, and number theory), and origins of falsehood (including violations of common sense, insufficient information, mathematical contradictions, and many others). Initially, we enlisted participants from the American high school math competition (AMC) to manually generate these problems. However, this approach resulted in a dataset that was disproportionately skewed toward certain mathematical categories and specific types of falsehoods. Creating a balanced and comprehensive false math problem dataset proved to be a creative and complex task.

To address this challenge, we switched to LLMs and developed a pipeline that leverages them to convert valid problems from the MATH dataset \citep{hendrycks2021measuring} into false ones. The pipeline then conducts self-checks for falseness, complemented by human annotators to verify the authenticity of the false math problems. This process generated 2,000 potential false math problems, of which 635 were voted as false by the LLMs. Human annotators further scrutinized these, confirming 363 as genuinely false math problems. This curated dataset now serves as a vital tool for rigorously testing LLMs in a domain where their capabilities remain largely unproven.

We conducted an extensive evaluation of ten popular LLMs, ranging from open-source to specialized mathematical models, on the dataset. Our findings revealed significant limitations: the best-performing model, Gemini 1.5 Pro, correctly identified only 33.33\% of these problems. This highlights a broader issue with LLMs—while effective at solving well-defined problems, they struggle to identify inconsistencies and logical flaws, often rushing to incorrect conclusions. 

Our evaluation of LLMs on false math problems yielded several other key findings:
(1) Humans outperformed LLMs, achieving an average accuracy of 21.33\% compared to 19.72\%, indicating that humans are better at identifying subtle inconsistencies.
(2) As anticipated, simpler problems were generally easier for the models to identify, but they struggled significantly with more complex categories such as Geometry, Mathematical Contradiction, and Mathematical Invalidity, where accuracy often fell below 50\%.
(3) LLMs exhibited notable gaps in logical reasoning when step-by-step analysis was not enforced.
(4) LLMs were vulnerable to misleading hints, with even top models like Gemini and GPT-4 being easily influenced by false hints, highlighting a significant confirmational bias.
(5) Lastly, when LLMs correctly identified false problems, models like Gemini and Qwen-1.5 consistently provided accurate explanations, demonstrating their capacity to articulate reasoning effectively when detecting falsehoods.
These findings highlight the nuanced challenges LLMs face and suggest areas for potential improvements in their logical reasoning capabilities.

Overall, this study goes beyond merely identifying the weaknesses of LLMs; it lays the groundwork for future advancements. The major contributions of this paper are:
\begin{enumerate}
\item Introducing a new task, the False Math Problem.
\item Creating a balanced dataset of 363 verified false math problems.
\item Evaluating state-of-the-art LLMs on this new task, leading to noteworthy insights into their capabilities and limitations.
\end{enumerate}



% % \title{Evaluating Large Language Models on Identifying False Math Problems}

% The profound insight of Alfred North Whitehead, who declared that ``the science of pure mathematics, in its modern developments, may claim to be the most original creation of the human spirit," beautifully encapsulates the quintessential role of mathematics in the scaffolding of logical reasoning \cite{whitehead1911}. This foundational link between mathematics and logic sets the stage for examining the capabilities of modern Large Language Models (LLMs). While these AI systems have emerged as generative marvels, transforming numerous domains from natural language processing to complex problem-solving, their capacity for logical reasoning—especially in identifying inherently unsolvable mathematical problems—remains an area ripe for exploration. This research delves into this critical aspect, assessing how LLMs handle the challenge of discerning false math problems, thereby probing the limits and potential of their logical faculties. 



% A math problem is considered false and unsolvable if no solution exists without modifying the problem statement (e.g., figure \ref{fig:false_math_problem_example}). Human beings can often discern the solvability of a math problem based on their mathematical knowledge and intuition. This research aims to evaluate the performance of LLMs in recognizing false math problems, providing insights into their limitations and potential areas for improvement.


% Recent studies have demonstrated the prowess of LLMs like GPT-3 and GPT-4 in generating and solving complex mathematical problems \cite{brown2020language, openai2023gpt4}. These models have shown exceptional accuracy in providing solutions to well-posed problems. However, the challenge of identifying false math problems poses a unique test of their reasoning abilities. Our project seeks to fill this gap by systematically evaluating the performance of popular LLMs in detecting unsolvable math problems.
% \begin{figure}[t]
% \centering
% \includegraphics[width=1.0\columnwidth]{figures/false_math_example_from_dataset.pdf} 
% \caption{Example of a ``False Math Problem" from our dataset. The model responses are their final numerical output after reasoning.}.
% \label{fig:false_math_problem_example}
% \end{figure}
% To conduct this evaluation, we first created a dataset of false math problems. Using GPT-4, we generated raw false math problems by altering valid problems sourced from the MATH dataset \cite{hendrycks2021measuring}. GPT-4 was instructed to provide explanations for why these problems were unsolvable. Following an automated filtering process of 2000 raw false math problem, human verification was conducted on 635 automatically generated problems, resulting in the identification of 363 genuine false math problems. 
% % and 272 problems that were still solvable. 
% This dataset serves as a critical resource for testing the diagnostic capabilities of LLMs in mathematics.

% In our experiments, we tested ten popular LLMs on the dataset of false math problems. The results revealed that the best-performing model, Gemini 1.5 Pro, identified only 121 false problems (33.33\%). This highlights a significant shortcoming of current LLMs: their inability to consistently recognize unsolvable problems. While LLMs excel at solving well-defined problems, they often fail to detect inconsistencies or errors in problem statements, quickly converging on incorrect solutions.

% Moreover, our dataset creation process underscores the difficulty LLMs face in generating false math problems. Despite instructions to create unsolvable problems, 42.8\% of the generated problems were still solvable. This finding suggests that LLMs have an inherent bias towards generating coherent and solvable outputs, even when tasked with creating flawed problems.

% Furthermore, we have posed five key research questions surrounding LLMs' capacity in identifying false math problems. We conducted several experiments to present their weakest mathematical topics, their ability to identify false math problems with different instructions, their confirmational-bias, and few other important aspects. 

% % The implications of our study are twofold. Firstly, it calls attention to a critical weakness in current LLMs, suggesting the need for improved training and evaluation methodologies to enhance their diagnostic capabilities. Secondly, it provides a valuable dataset for future research, enabling the development of more robust models capable of recognizing and handling unsolvable math problems. By addressing these challenges, we can pave the way for more reliable and versatile AI systems in the field of mathematical problem-solving. The major contributions of this paper are:
% % \begin{enumerate}
% %     \item We proposed a new task, False Math Problem, and generated a dataset of 363 verified false math problems, sourced and altered from the MATH dataset using GPT-4 and human verification, to evaluate LLMs' capabilities in identifying false math problems.
% %     \item We tested state-of-the-art LLMs on this dataset revealed that the best model, Gemini 1.5 Pro, identified only 33.33\% of the false problems, highlighting a significant shortcoming in current LLMs.
% %     \item We showed that LLMs have an inherent bias towards generating solvable math problems, even when tasked with creating unsolvable ones, indicating a need for improved training.
% %     \item We posed critical research questions regarding LLMs' ability to identify false math problems, exploring their weaknesses and confirmational biases.
% % \end{enumerate}

% The key implications of our study highlight a critical weakness in current LLMs, emphasizing the need for improved training and evaluation methodologies, and provide a valuable dataset for future research in mathematical problem-solving. Surrounding these matters, the major contributions of this paper are as follows:

% \begin{enumerate}
%     \item Proposing a new task, False Math Problem, and generating a dataset of 363 verified false math problems, sourced and altered from the MATH dataset using GPT-4 and human verification.
%     \item Testing state-of-the-art LLMs on this dataset, revealing that the best model, Gemini 1.5 Pro, identified only 33.33\% of the false problems, highlighting a significant shortcoming in current LLMs.
%     \item Demonstrating that LLMs have an inherent bias towards generating solvable math problems, indicating a need for improved training.
%     \item Posing critical research questions regarding LLMs' ability to identify false math problems, exploring their weaknesses and confirmational biases.
% \end{enumerate}



==> 2Related_Work.tex <==
                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                % Written by Junyi (Related Work)
\section{Related Work}

Mathematical reasoning has long been a significant area of focus in artificial intelligence research. One of the pioneering works in automatic math word problem (MWP) solving \citep{bobrow1964question} developed a system that used rules and a parser to translate word problems into algebraic equations for computational solving.
With the advent of deep learning, Seq2Seq models \citep{wang2017deep,huang2018neural,saxton2018analysing,wang2019template,xie2019goal,liang2022mwp} and Seq2Tree \citep{wang2018translating,liu2019tree,wu2020knowledge} models began leveraging neural network architectures to process and solve complex mathematical problems, laying the foundation for further advancements in the field. 
Recently, we have witnessed the development of general purpose LLMs such as GPT-4\citep{achiam2023gpt}, Claude3\citep{anthropic2024claude}, Gemini\citep{reid2024gemini}, Llama3\citep{meta2024llama3} and etc. Mathematical reasoning benchmarks GSN8K\citep{cobbe2021training} and MATH \citep{hendrycksmath2021}, has become crucial in the evaluation of fundamental reasoning and cognitive capabilities of LLMs, ensuring they can handle sophisticated mathematical reasoning and problem-solving tasks effectively.
On the other side, there are specific LLMs trained on mathematical corpora \citep{azerbayev2021llemma,wang2023generative,paster2023openwebmath,toshniwal2024openmathinstruct}, including MathVerse\citep{lewkowycz2022solving}, Internlm-Math\citep{ying2024internlm} and DeepSeekMath\citep{shao2024deepseekmath}.


Several techniques have been developed to improve the mathematical reasoning capabilities of LLMs. Prompt engineering, including zero-shot and few-shot learning \citep{brown2020language,lewkowycz2022solving}, involves designing specific prompts to guide the model to produce more accurate and contextually relevant outputs. Chain-of-thought (CoT) prompting \citep{wei2022chain} is another technique that involves converting a query into a set of intermediate queries in a sequential manner to enhance the reasoning process of LLMs. Deeply Understanding the Problems (DUP) \citep{zhong2024achieving} emphasizes a thorough comprehension of the problem before attempting to solve it, ensuring that the nuances and complexities are fully grasped. Program-aided language modeling \citep{zhou2023solving,zhang2024evaluating,ying2024internlm} leverages the code completion capabilities of language models to enhance their reasoning capacities, as demonstrated in recent studies. Agent-aided approaches \citep{lei2024macm,toshniwal2024openmath}, including multi-agent techniques, collectively contribute to significant improvements in the mathematical reasoning and problem-solving abilities of modern LLMs.


==> 3Dataset_Creation.tex <==
\section{Dataset Creation}

Generating false math problems is not only inherently a creative process, but it is also unconventional, as it is not a typical human task.
Our initial approach involved enlisting American high school math competition (AMC) participants to create false math problems from scratch. However, this effort resulted in a problem set that is biased toward particular mathematical categories and specific types of falsehoods. We then explored data augmentation via LLMs, using this seed dataset created by humans, but this approach also failed. Inspired by recent studies on generating synthetic data using LLMs \citep{Eldan2023,Li2023,Yuan2023}, we extensively experimented with modifying valid problems from the MATH dataset using GPT-4 by giving it well-crafted prompts. This approach significantly improved the likelihood of generating genuinely false math problems.
We began by generating a pool of raw false math problems using GPT-4. After a carefully designed filtering process conducted by GPT-4, human evaluators assessed the falsehood of these problems. The entire process is summarized in Figure \ref{fig:dataset_creation}, with details provided in the following sections.

%False math problem generation is undoubtedly a creative process. Initial attempts to create false math problems involved enlisting American high school math competition (AMC) participants to generate these problems from scratch. However, their efforts often resulted in problems that were either solvable, too simple, or followed repetitive patterns. Later, we tried data-augmentation via GPT-4 using seed dataset but it also tended to generate solvable problems when tasked with creating false problems directly. Recognizing these challenges, we shifted our approach to modifying valid problems from the MATH dataset using GPT-4, which significantly improved the likelihood of generating genuinely false math problems. Recent studies have also relied on the creativity of LLMs to curate challenging datasets \cite{Eldan2023,Li2023,Yuan2023}, which pushed us further to follow suit. Even though our dataset creation process relies upon LLMs, we did not rely too heavily on it. We first generated a pool of raw false math problems from LLMs, and after a filtering process we had human evaluators judge the falsehood of those problems. The entire process is summarized in figure \ref{fig:dataset_creation}, while the details is laid out below.

\begin{figure*}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{figures/dataset_creation_figure_v3.pdf} 
\caption{False Math Problem (FMP) dataset creation process}
\label{fig:dataset_creation}
\end{figure*}

\subsection{Valid to Raw False Math Problem}
To compile a diverse collection of false math problems across different categories (e.g., Algebra, Geometry), we used the MATH dataset \citep{hendrycks2021measuring} as our source for valid problems. We selected 400 problems from each of five categories—Algebra, Geometry, Counting \& Probability, Number Theory, and Precalculus—totaling 2,000 valid problems. Given its creativity and strong performance on the MATH dataset, we chose GPT-4 as our LLM for this task.

We provided GPT-4 with each valid math problem and its correct solution, instructing it to convert the problem into a false and unsolvable version. Additionally, we asked GPT-4 to include a brief explanation of why the problem is false—a crucial step that significantly improved the generation of genuinely false problems.

\subsection{Automatic Filtration \& Human Verification}
We found that many of the 2,000 generated false math problems were actually solvable, so we implemented a clever self-evaluation process to filter out those that did not meet the criteria for being truly unsolvable.

In this self-evaluation process, GPT-4 was initially presented with a ``raw false math problem" to solve. After providing a solution, it was prompted with a ``simple explanation" of why the problem was unsolvable, encouraging GPT-4 to reflect on its initial solution. Finally, we posed a multiple-choice question to GPT-4, asking for its final decision on the entire conversation. The choices (A, B, or C) are outlined in Figure \ref{fig:dataset_creation}.

If GPT-4 outputs ``A", it implies that GPT-4 believes the raw false math problem to be a genuine false math problem but not a challenging one to identify. If GPT-4 outputs ``B", it implies that GPT-4 considered the raw false math problem to be a genuine false math problem and a challenging one that it could not identify to be false when initially presented. An output of ``C" implies that the false math problem is a valid math problem with a possible solution.

We filtered out the problems marked ``C" and ``A," as they had a lower likelihood of being genuine and challenging false math problems. This left us with 635 problems, which were then reviewed by human annotators for verification. Each annotator independently assessed all 635 problems to determine whether they were genuinely false, meaning no solution existed as presented. Through this manual verification process, 363 problems were confirmed as genuine false math problems by both annotators. The other 272 problems were found to be solvable and were discarded. 

% Written by Junyi (Dataset Statistics)
\subsection{Dataset Statistics}

Figure \ref{fig:dataset} (left) illustrates the distribution of false math problems across various mathematical categories, demonstrating GPT-4's balanced capability in generating false math problems for each category. A notable trend within the dataset is the prevalence of higher-difficulty problems, indicating that more complex math problems are more likely to mislead GPT-4 when transformed into false problems.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/dataset.pdf}
    \caption{Distributions of the dataset by difficulty level and math category (Left); by origin of falsehood (Right).}
    \label{fig:dataset}
\end{figure}

To understand the origins of errors in the dataset, we randomly selected 50 samples and manually classified the types of falsehoods. Subsequently, we used GPT-4o to systematically categorize each false problem into these predetermined categories. As shown in Figure \ref{fig:dataset} (right), the analysis reveals that Mathematical Contradiction and Invalidity are the most common types of errors generated by GPT-4. This trend suggests that the model tends to introduce these specific errors during the problem conversion process because these two types are easier to construct and are applicable across various problems. Additionally, these types of errors are more likely to be retained as they effectively challenge the model's problem-solving accuracy. In contrast, errors such as Common Sense Violation, Misleading Statements, and Undefined Terms occur less frequently, showcasing the model's preferences in generating false math problems. The analysis highlights the model's ability to generate complex false problems and its tendency towards certain types of errors, showcasing both the strengths and preferences of the model.

==> 4Evaluation_Method.tex <==
\section{Evaluation Method}
The primary task for LLMs in this research is to determine whether they can identify issues in given false math problems. However, directly asking this question would signal to the LLMs that the problem is false, thereby influencing their response. The same constraint applies to human annotators; we cannot explicitly ask whether the questions are false. Instead, we ask them to solve the problems without providing any hints. By analyzing their solutions, we can determine whether the falsehood was detected. For instance, if a solution mentions that the problem is solvable only with additional constraints, it indicates awareness of the issue. Consequently, evaluating the LLMs' responses to false math problems requires careful and nuanced assessment.

%The LLM responses are not single numerical answers to the problems. Instead, the responses are generally broad, and the identification of the falsehood in the problem occurs at random points within their responses, with the language used to indicate it varying widely—sometimes pointing out a misunderstanding, noting an inconsistency, or identifying other issues in the problem statement. As a result, the evaluation is not straightforward and involves careful consideration and examination of the LLM's response to determine whether it completely ignored the falsehood in the math problem.

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.7\columnwidth]{figures/confusion_matrix.pdf} 
% \caption{Confusion matrix for false math problem evaluation.}.
% \label{fig:confusion_matrix}
% \end{figure}

%While human evaluation is considered the gold standard, it is time-consuming and cost-inefficient. 
%To solve this tricky problem, we aim to implement an accurate automatic evaluation process by an LLM. To obtain the best LLM and associated prompts to do the evaluation, we first decide a golden evaluation standard by human and then try out different auto-evaluation prompts. To obtain the gauge standard, we selected GPT-4-Turbo (2024-04-09 Update) as our inferred LLM ($LLM_i$), and two PhD-level reviewers evaluated its responses to the dataset. Checking the solutions provided by $LLM_i$ to the genuine false math problems, the reviewers agreed that for 300 of these problems, $LLM_i$ failed to identify any issue with the problem statements, effectively being tricked by the false problems. This resulted in a gold-standard accuracy of 17.36\% (63 out of 363 identified) for $LLM_i$. The same responses from $LLM_i$ were then evaluated by two automatic evaluator LLMs ($LLM_e$) using different prompting techniques and compared with the gold-standard evaluation. GPT-4 and GPT-4o were used as $LLM_e$.

To address this challenge, we aimed to implement an accurate automatic evaluation process using an LLM. We first established a gold standard by having two PhD-level reviewers evaluate responses from GPT-4-Turbo (2024-04-09 Update) on the dataset. The reviewers found that GPT-4-Turbo failed to identify issues in 300 of the 363 genuine false math problems, achieving a gold-standard accuracy of 17.36\% (63 out of 363 identified). We then tested different auto-evaluation prompts with two other LLMs, GPT-4 and GPT-4o, comparing their performance against the gold standard. We use $LLM_i$ to denote the target LLM to be evaluated and $LLM_e$ to denote the candidate LLM as an evaluator. 

% Therefore, we used GPT-4 as the automatic evaluator for this task. Nevertheless, to gauge how efficient the automatic evaluation with GPT-4 is, we performed human-evaluation for one LLM's inference and compared it against the automatic evaluation method using two different versions of GPT-4 and various prompting techniques. The best prompt and GPT-4 version was chosen for the automatic evaluator for all the other LLMs in our experiments.

% During our dataset creation process, our two PhD-level reviewers also evaluated GPT-4 Turbo's (2024-04-09 Update) responses on the false math problem dataset. Among the 363 genuine false math problem, our annotators mutually agreed that for 300 of those problems, GPT-4-Turbo could not identify any issue with the problem statement, in other words, were tricked by the false math problems. This results in a gold-standard human-evaluation of 17.36\% (63 out of 363 identified) on the dataset for GPT-4 Turbo. Maintaining this human-evaluation as the ground truth, we compared different prompting techniques on GPT-4 and GPT-4o for automatic evaluation.

\input{tables/tab_automatic_evaluation_method_performance}
 
\subsection{Auto-Evaluation Prompts}
For the automatic evaluation with $LLM_e$, we tried the following prompting techniques:
\begin{itemize}
    \item Simple Prompt: Problem X: {[`False Math Problem’]}
LLM Y’s Solution: {[`$LLM_i$ Solution’]}
Problem X is a false math problem and cannot be solved without modifications to the problem statement. Did LLM Y identify this in its solution?
Please answer `Yes' or `No'.
    \item Simple Prompt + Explanation: Insert ``Why Problem X is a False and Unsolvable Math: {[`Simple Explanation']}" right after the LLM Y's Solution.
    \item Chain-of-thought prompt: Provide one positive and one negative example, and explain step by step how the LLM Y identified or missed the falsehood of the math problem. Here, instead of answering ``yes" or ``no" directly, we prompted it to reason, and finally answer.

\end{itemize}

\input{tables/tab_main_results_gpt4}

As a binary classification task with human-evaluation as the gold-standard (Positive: Correctly identified the false math problem; Negative: Did not identify the false math problem), the confusion matrix elements (TP, TN, FP, FN) are defined by the agreement between the auto-evaluation and the human evaluation. 
% \begin{itemize}
%     \item True Positive: Auto-Evaluation says LLM has identified, and human-evaluation agrees.
%     \item False Positive: Auto-Evaluation says LLM has not identified, and human-evaluation disagrees.
%     \item True Negative: Auto-Evaluation says LLM has NOT identified, and human-evaluation agrees.
%     \item False Negative: Auto-Evaluation says LLM has NOT identified, and human-evaluation disagrees.
% \end{itemize}

Here, we look at the F1 Measure, Accuracy, and the performance of $LLM_i$ using $LLM_e$ compared to human evaluation. The evaluation by $LLM_e$ is defined as the percentage of false math problems identified by $LLM_i$ (True Positives + False Positives). From Table \ref{table:auto_evaluation_performance}, we observe that the ``Simple Prompt + Explanation" with GPT-4 as $LLM_e$ achieves the highest accuracy. However, the ``Simple Prompt" with GPT-4 performs best across all metrics and aligns most closely with human evaluation. Therefore, we selected the ``Simple Prompt" with GPT-4 as our automatic evaluator for the false math problem dataset across all LLMs in subsequent experiments.


==> 5Experiments.tex <==
\section{Experiments}

% Written by Junyi (Large Language Models)
\subsection{Large Language Models}
In this paper, we evaluate state-of-the-art LLMs renowned for their performance on the MATH dataset. We selected GPT-4, Claude 3 Opus, and Gemini 1.5 Pro among closed-source LLMs for their superior handling of complex mathematical tasks. We also included math-specific LLMs, DeepSeek Math RL and InternLM2-Math, designed for mathematical reasoning. Additionally, we assessed open-source LLMs like Llama 3 70B, Yi 1.5 34B, Mixtral 8x 22B, Qwen 1.5 72B, and DeepSeek v2, each offering unique strengths in reasoning and problem-solving. This selection aims to be comprehensive and representative.

% Written by Junyi (Experimental Setup)
\subsection{Experimental Setup}
In our experiments, we employed the greedy decoding strategy for all LLMs. We accessed the capabilities of the closed-source models via APIs. For the open-source models, we utilized the Hugging Face library on A100 GPUs to ensure optimal configuration. For other settings, including system prompts, we adhered strictly to the configurations specified in the respective models' papers or technical reports.

% Written by Junyi (Primary Experiment)
\subsection{Results and Discussions}
We introduce our results in the context of our research questions and discuss our main findings.

\subsubsection{Q0: How do the LLMs perform in the false math problem challenge?}

In Table \ref{table:model_evaluation}, we illustrate the LLMs' performance on the MATH \citep{hendrycksmath2021} dataset (MATH-Perf), as reported by their papers or technical reports, the number of false math problems correctly identified (\# Identified FMP), and the accuracy of these identifications using the auto-evaluation method. The results highlight that the Gemini-1.5-Pro model outperformed others, correctly identifying 121 false problems with an accuracy of 33.33\%. Following closely were GPT-4, Qwen-1.5, and Claude-3, each demonstrating strong performance. However, models such as Llama-3, Yi-1.5, and the two math-specialized LLMs, Deepseek-Math-7B-RL and Internlm2-Math-20B, significantly underperformed in the accuracy of identifying FMPs. These findings underscore that strong performance on general math datasets does not necessarily translate to high effectiveness in identifying false math problems, suggesting that different skill sets are required for general mathematical reasoning versus falsehood detection in specialized tasks.

% Written by Junyi (Reasearch Questoin Q1)
\subsubsection{Q1: What types and origins of false math questions pose the greatest challenges for LLMs?}

\subsubsection{Analysis by difficulty level and mathematical category}

We conducted an in-depth analysis of the fine-grained accuracy of the top three performing LLMs (Gemini, GPT-4, Qwen1.5) across various difficulty levels (ranging from level 1 to level 5) and mathematical categories (such as Algebra, Counting \& Probability, etc.), as illustrated in Figure \ref{fig:acc_per_level_per_category}.

From the average accuracy of the top three LLMs (top-left), it is evident that the performance in identifying false math problems is slightly higher for simpler to moderately difficult problems (levels 1-3) compared to more challenging ones (levels 4-5). Particularly, compared to GPT-4 and Qwen1.5, Gemini exhibits a notable strength in this aspect. When evaluating by mathematical category, Algebra demonstrates the highest accuracy, followed by Number Theory, with Geometry being the most challenging, evidenced by an average accuracy of only 23\%.

A comparative analysis of the performance of the top three LLMs in different mathematical categories reveals varied strengths among the models. Gemini excels in Algebra and Number Theory, GPT-4 performs best in Counting \& Probability and Number Theory, while Qwen1.5 shows superior performance in Algebra and Precalculus. Conversely, GPT-4 exhibits significant deficiencies in Geometry, and Qwen1.5 struggles with Counting \& Probability and Geometry. Notably, Gemini does not exhibit substantial weaknesses in any particular category.

% \begin{figure*}[!htbp]
%     \centering
%     \includegraphics[width=\textwidth]{figures/acc_per_level_per_category_5.pdf}
%     \caption{Accuracy heatmaps for different difficulty levels and categories. Top-left: Average accuracy of top 3 LLMs. Top-right: Gemini-1.5-Pro (Rank 1). Bottom-left: GPT-4 (Rank 2). Bottom-right: Qwen1.5-72B (Rank 3).}
%     \label{fig:acc_per_level_per_category_1}
% \end{figure*}


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/acc_per_level_per_category.pdf}
    \caption{Accuracy heatmaps for different difficulty levels and categories. Top-left: Average accuracy of top 3 LLMs. Top-right: Gemini-1.5-Pro (Rank 1). Bottom-left: GPT-4 (Rank 2). Bottom-right: Qwen1.5-72B (Rank 3).}
    \label{fig:acc_per_level_per_category}
\end{figure}

\subsubsection{Analysis by origin of falsehood and mathematical category}

We investigated the fine-grained accuracy of the top three LLMs across different origins of falsehood and mathematical categories, as depicted in Figure \ref{fig:acc_per_falsehood_per_category}.

From the average accuracy of the top three LLMs, it is shown that they have slightly higher accuracy in identifying false math problems stemming from Insufficient Information and No Solution categories. In two sample-heavy falsehood categories (Mathematical Contradiction and mathematical Invalidity), accuracy is notably lower in Counting \& Probability and Geometry, indicating that the main reason for lower performance in these categories is the LLMs' difficulty in recognizing mathematical contradictions and invalidity.

A horizontal comparison among the top three LLMs reveals distinct performances: GPT-4 achieves 0\% accuracy in common sense violations, Gemini and GPT-4 both struggle with Undefined Terms, achieving 0\% accuracy, whereas Qwen1.5 attains a 50\% accuracy rate in this category. Qwen1.5, however, shows a 0\% accuracy rate in Misleading Statements, while Gemini significantly outperforms the other two in the Insufficient Information category. In the most populated classes, Mathematical Contradiction and Mathematical Invalidity, all three LLMs exhibit comparable performance.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/acc_per_falsehood_per_category.pdf}
    \caption{Accuracy heatmaps for different origins of falsehood and categories. `-' indicates no samples in the cells.}
    \label{fig:acc_per_falsehood_per_category}
\end{figure}


This analysis underscores the differential capabilities and limitations of each LLM across various mathematical domains, revealing that most fine-grained accuracies are below 50\%. These findings indicate that there is significant room for improvement in the task of identifying false math problems, highlighting the need for further enhancement of LLM performance in this area.


\subsubsection{Q2: How does LLM performance compare to human performance in identifying false math problems without any hints?}

This question seeks to compare the effectiveness of LLMs and humans in identifying false math problems when no additional hints or guidance are provided. To that end, we recruited 15 graduate-level students to participate in our study.
For this human benchmarking stage, we needed to ensure that the human participants did not get any hints that the problems were false math problems to keep their responses unbiased. The participants were provided with the false math questions and asked to write down their responses. 

Each participant was given 10 problems from our dataset to solve within 72 hours. They were strictly prohibited from using any AI tools. The participants were asked to solve 10 problems, not all 363 problems, for two main reasons. Firstly, to reduce their effort and prevent fatigue-induced errors. Secondly, to prevent students from identifying that there is a prominent pattern (all mathematical questions are false and unsolvable) in the questions they were facing. The students' responses were manually evaluated by the same evaluators that evaluated GPT-4's responses in our auto evaluation-method step to keep the evaluation consistent. We observed an average accuracy of 21.33\% in identifying false math problems by the human participants. This performance is 1.6\% more than the average of our 10 LLMs, which is 19.72\% (table \ref{table:model_evaluation}). Even though the performance gap is small, it suggests that this task is comparatively easier for human beings than LLMs. However, we also need to address that this is not an apple-to-apple comparison. LLMs were solving one problem at a time whereas the human participants had 10 questions to sense a pattern of falsehood. Due to input-window limitation, we cannot expect LLMs to reason through even two questions in many cases, let alone 10. On the other hand, a single LLM, arguably, has in its possession more mathematical knowledge than a graduate-level student; what we have observed is the failure to reason from them better than humans.

\subsubsection{Q3: How do the LLMs react when they are asked to simply output ``Yes" or ``No"?}
Traditional NLP tasks evaluate systems based on explicit task instructions, where the system knows the evaluation criteria. For example, in machine-translation tasks, if the instruction is to translate ``Gracias" from Spanish to German, a correct response would be ``Danke." In contrast, if the instruction changes to: ``Translate the following \textit{English} to German: `Gracias'", a correct response would clarify that ``Gracias" is Spanish, not English, and then provide the German equivalent, ``Danke." Essentially, evaluating the system based on the acknowledgement of the underlying issue in the task instruction is something novel we have done in our primary experiment, Q0. We can consider Q0 as an ``Evaluation-unaware" experiment where the system is not aware of the falsehood in the task instruction and not aware that it will be evaluated based on the identification of such falsehood. For Q3, we want to test what happens when the system \textit{is} aware of the possibility of the falsehood.
\input{tables/tab_task_aware_results}

The prompt for this ``Evaluation-aware" experiment was ``Is the above math problem a false and unsolvable math problem? Output `Yes' if it is, `No' otherwise.". Since LLMs tend to have a bias towards always outputting ``Yes" or ``No," we flipped the statement to force the LLMs to choose logically in another round of experiments with the following prompt. ``Is the above math problem a valid and solvable math problem? Output `Yes' if it is, `No' otherwise." Notice how, for the same sample in the dataset, we expect the LLM to respond in ``Yes" in one and ``No" in another. The results are detailed in table \ref{table:yes_no_task_aware}. We can observe that, the contrast between switching ``Yes" and ``No" is very high in some LLMs. This adds to the notion that some of the LLMs have a high bias towards selecting ``Yes" or ``No" and their mathematical reasoning capacity without step-by-step generative approach is very weak.
\input{tables/tab_hint_based_prompt}

\subsubsection{Q4: How likely can the LLMs' discriminative capability be misled by false Hints?}
Aside from Evaluation-aware and unaware task instructions, we can also test the LLMs' decisive integrity by misleading them with faulty hints. To that end, we conduct this experiment where, in one round, we provide a true hint to the LLM that the problem can be a false and unsolvable math problem, and in another round, we provide a misleading hint that the problem is a valid and solvable math problem whereas they are not. From table \ref{table:hint_based_experiments}, we can infer that while LLMs score high when it has true hints, they get easily misled by the false hints. The LLMs in this experiment exhibited high confirmational-bias, where they agree to the instruction easily, without rationalizing and reaching a different conclusion.

% Written by Junyi (Reasearch Questoin Q5)
\subsubsection{Q5: How accurate are the explanations provided by LLMs when identifying false math problems?}

To deepen our understanding beyond binary performance evaluation, we investigate the correctness of LLMs' explanations when 
they identify a math problem as false. Specifically, we selected the top three LLMs and examined 21 samples, which all three LLMs correctly identified as false. Our analysis involved two rounds of manual verification. The first round ensured that all selected samples were indeed correctly identified as false, and the second round focused on assessing the correctness of the explanations provided. Our findings revealed that both Gemini and Qwen1.5 provided accurate explanations for all 21 samples (21/21), while GPT-4 offered correct explanations for 20 out of 21 samples (20/21). These results suggest that when an LLM identifies a math problem as false, its explanation is generally reliable.

==> 6Conclusion.tex <==
\section{Conclusion}
This study explores the ability of LLMs in identifying false and unsolvable mathematical problems, revealing notable limitations in their logical reasoning. A major contribution of this paper is the creation of a dedicated dataset of false math problems, which serves as a crucial resource for evaluating and improving LLMs. Despite their success in solving complex math problems, models like GPT-4 and Gemini 1.5 Pro struggled with discerning unsolvable problems, with the top-performing model correctly identifying only 33.33\% of false problems in the dataset. Performance varied across different mathematical categories and types of falsehoods, with Geometry and Mathematical Contradictions posing the greatest challenges. Additionally, LLMs exhibited high confirmation bias and were easily misled by false hints, indicating the need for improved training in handling deceptive instructions. Comparisons with human performance, further highlight the current shortcomings of LLMs in this area. While LLMs provided reliable explanations when correctly identifying false problems, there is room for improvement in their explanatory capabilities. The findings underscore the necessity for refining LLM training methodologies and prompt design to enhance their reliability and versatility in mathematical problem-solving, paving the way for more robust AI systems.

==> tables/tab_automatic_evaluation_method_performance.tex <==
\begin{table}[htbp]

\centering
\small
\begin{tabular}{lcccc}
\hline\\ [-1.5ex]
\vspace{0.1cm}\textbf{Prompt} & \textbf{LLM\(_{e}\)} & \makecell{\textbf{Acc}} & \makecell{\textbf{F1}} & \makecell{\textbf{Eval}}\\
\hline\\[-1.5ex]
\vspace{0.1cm}\makecell[l]{Human-Evaluation\\(Gold Standard)} & - & 100 & 100 & 17.36\\
\\[-1.5ex]
\vspace{0.1cm}\makecell[l]{Simple Prompt} & GPT-4o & 85.67 & 61.79 & 4.68 \\
\\[-1.5ex]
\vspace{0.1cm}\makecell[l]{Simple Prompt\\ + Explanation} & GPT-4o & 84.02 & 59.26 & 3.58 \\
\\[-1.5ex]
\vspace{0.1cm}\makecell[l]{Chain-of-thought} & GPT-4o & 85.95 & 64.57 & 4.96 \\
\\[-1.5ex]
\vspace{0.1cm}\makecell[l]{Simple Prompt} & GPT-4 & 88.15 & \textbf{80.44} & \textbf{19.83} \\
\\[-1.5ex]
\vspace{0.1cm}\makecell[l]{Simple Prompt\\ + Explanation} & GPT-4 & \textbf{89.81} & 77.99 & 9.37\\
\hline
\end{tabular}
\caption{Automatic-Evaluation Methods' performance considering Human-Evaluation as the ground truth. Inferred model: GPT-4-Turbo. Eval = the performance of GPT-4-Turbo using respective evaluation method.}
\label{table:auto_evaluation_performance}
\end{table}


==> tables/tab_hint_based_prompt.tex <==
\begin{table}[h!]

\centering
\small
\begin{tabular}{lccc}
\hline\\ [-1.5ex]
\vspace{0.1cm}\textbf{Model} & \textbf{True Hint} & \textbf{False Hint} & \textbf{Avg(\%)} \\
\hline\\ [-1.5ex]
Gemini-1.5-Pro & 95.87 & 33.61 & 64.74\\
Claude-3-Opus &  86.78 & 26.45 & 56.62 \\
Mixtral-8X22B-V0.1 &  75.21 & 30.30 & 52.75\\
Yi-1.5-34B & 70.52 & 24.52 & 47.52\\
Llama-3-70B &  79.06 &  13.77 & 46.42 \\
Qwen-1.5-72B & 63.36 & 28.65 & 46.00\\
GPT-4 & 63.36 & 28.10 & 45.73 \\
Deepseek-V2 &  64.19 & 22.59 & 43.39\\
Deepseek-Math-7B-RL &  69.42 & 9.37 & 39.40\\
\vspace{0.1cm}Internlm2-Math-20B &  58.95 & 10.19 & 34.57\\
\hline\\ [-1.5ex]
\end{tabular}
\caption{Performance (Accuracy) of various LLMs on prompts that contain hints. True Hint Prompt: ``Solve the above math problem. Hint: The problem can be a false and unsolvable math problem.". False Hint Prompt: ``Solve the above math problem. Hint: The problem is a valid and solvable math problem."}
\label{table:hint_based_experiments}
\end{table}


==> tables/tab_llms.tex <==
\begin{table*}[htbp]
    \caption{Comparison of selected state-of-the-art LLMs on Mathematical Reasoning.}

\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\textbf{LLM} & \textbf{\# Para} & \textbf{Purpose} & \textbf{Context Window} & \textbf{MATH} & \textbf{Techniques}\\
\hline
GPT-4 & - & General & 8k & 64.5\textsuperscript{\href{https://github.com/openai/simple-evals?tab=readme-ov-file}{1}} & (0-shot, CoT)\\
GPT-4 Turbo & - & General & 128k & 73.4\textsuperscript{\href{https://github.com/openai/simple-evals?tab=readme-ov-file}{1}} & (0-shot, CoT)\\
Gemini 1.5 Pro & - & General & 128k & 67.7 \cite{reid2024gemini}& (4-shot, Minerva
prompt)\\
Claude-3-opus & - & General & 200K & 60.1\textsuperscript{\href{https://www.anthropic.com/news/claude-3-family}{2}} & (0-shot, CoT)\\
Yi 1.5 & 34B & General & 4K & 50.1 &\\
Llama 3 & 70B & General & 8K & 50.4\textsuperscript{\href{https://ai.meta.com/blog/meta-llama-3}{3}} & (4-shot, CoT)\\
Qwen 1.5 & 72B & General & 32K & 40.6 &\\
Mixtral 8x22B & 39B/141B & General & 64K & 49.8 &\\
DeepSeek-V2 & 21B/236B & General & 128K & 53.9 &\\
DeepSeek-Math-RL & 7B & Math & 4K & 51.7 &\\
Internlm2-Math & 20B & Math & 4K & 37.7 &\\
\hline
\end{tabular}
\label{tab:llm_comparison}
\end{table*}

==> tables/tab_main_results_gpt4.tex <==
\begin{table*}[ht]

\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccccc}

\hline\\ [-1.5ex]
\vspace{0.1cm}\textbf{Model} & \textbf{Scope} & \textbf{Source} & \textbf{MATH-Perf (\%)} &\textbf{\# Identified FMPs} & \textbf{Accuracy (\%)} \\
\hline\\ [-1.5ex]
% GPT-4-Turbo & General & Closed & 72.6 & 72 & 19.83 (17.36) \\
Gemini-1.5-Pro & General & Closed & 58.5 & 121 & 33.33 \\
GPT-4 & General & Closed & 52.9 & 114 & 31.40 \\
Qwen-1.5-72B & General & Open & 41.4 & 107 & 29.48 \\
Claude-3-Opus & General &  Closed & 60.1 & 101 & 27.82 \\
Mixtral-8X22B-V0.1 & General & Open & 41.8 & 86 & 23.69 \\
Deepseek-V2 & General & Open & 43.6 &  63 & 17.36 \\
Yi-1.5-34B & General & Open & 50.1 & 43 & 11.85 \\
Deepseek-Math-7B-RL & Math & Open & 51.7 & 37 & 10.19 \\
Llama-3-70B & General &  Open & 50.4 &  26 & 7.16 \\
\vspace{0.1cm}Internlm2-Math-20B & Math & Open & 37.7 &  18 & 4.96 \\
\hline
\end{tabular}
\caption{This table presents the performance of various LLMs on the False Math Problem dataset (N = 363). It reports the number of problems each model correctly identified as false. Auto-evaluation model: GPT-4.}
\label{table:model_evaluation}
\end{table*}


==> tables/tab_main_results_gpt4o.tex <==
\begin{table}[h!]
\caption{This table presents the auto-evaluation performance of various LLMs on the False Math Problem dataset (N = 363). The table reports the number of problems each model correctly identified as false. Auto-evaluation model: GPT-4o. For GPT-4 Turbo the metric in the parantheses represents the human-evaluation.}
\centering
\begin{tabular}{lccc}
\hline
\textbf{Model} & \textbf{Decoding Strategy} & \textbf{Identified False Math} & \textbf{Accuracy (\%)} \\
\hline
Gpt 4 Turbo 2024 04 09 & Greedy & 13 & 3.58 (17.36) \\
Claude 3 Opus 20240229 & Greedy & 35 & 9.64 \\
Deepseek Math 7B Instruct & Greedy & 11 & 3.03 \\
Deepseek V2 & Greedy & 24 & 6.61 \\
Gemini 1.5 Pro & Greedy & 41 & 11.29 \\
Internlm2 Math 20B & Greedy & 15 & 4.13 \\
Meta Llama 3 70B Instruct & Greedy & 17 & 4.68 \\
Mixtral 8X22B Instruct V0.1 & Greedy & 30 & 8.26 \\
Qwen1.5 72B Chat & Greedy & 18 & 4.96 \\
Yi 1.5 34B Chat & Greedy & 21 & 5.79 \\
\hline
\end{tabular}

\label{table:model_evaluation}
\end{table}


==> tables/tab_task_aware_results.tex <==
\begin{table}[h!]

\centering
\small
\begin{tabular}{lccc}
\hline\\ [-1.5ex]
\vspace{0.1cm}\textbf{Model}  & \textbf{Acc(\%)} & \textbf{Acc-S(\%)}  & \textbf{Avg(\%)}\\
\hline\\ [-1.5ex]
Gemini-1.5-Pro &  56.47 & 55.92 & 56.20 \\
GPT-4 & 25.07 & 39.94 & 32.51 \\
Claude-3-Opus &  29.20 & 22.31 & 25.76 \\
Llama-3-70B &  20.66 & 27.27 & 23.97 \\
Deepseek-V2 & 16.25 & 30.30 & 23.28 \\
Internlm2-Math-20B & 31.96 & 9.37 & 20.66 \\
Yi-1.5-34B & 22.87 & 11.02 & 16.94 \\
Mixtral-8X22B-V0.1 &  13.77 & 19.01 & 16.39 \\
Qwen-1.5-72B & 16.25 & 12.40 & 14.33 \\
\vspace{0.1cm}Deepseek-Math-7B-RL & 17.08 & 7.99 & 12.53 \\
\hline
\end{tabular}
\caption{The table presents the performance of various LLMs on Evaluation-Aware Task-Instructions that expect only ``Yes" or ``No" as outputs. The Acc-S column refers to prompts where ``Yes" and ``No" have been switched.}
\label{table:yes_no_task_aware}
\end{table}

